An Explicit Link between Extreme Value Theory and Compositional Data Analysis

Extreme value theory and compositional data analysis both study settings where relative information plays a central role. In multivariate extreme value theory, threshold exceedance limits satisfy homogeneity properties that separate the radial size of an extreme event from its relative profile. In compositional data analysis, positive vectors are analysed up to multiplicative scale, and inference is based on ratios or log-ratios between components. Consequently, both fields have developed several covariance and dependence representations of the underlying relative structure. In the H\"usler-Reiss model for extremes, these include variogram, covariance, and precision parametrizations. In compositional data analysis, analogous representations arise from pairwise log-ratios, centred log-ratios, and additive log-ratios. We establish an explicit link between the two fields that relates these different representations by a small set of simple transformations, including oblique projections, H\"usler-Reiss inverses, and the variogram map. From a methodological perspective, leveraging this algebraic connection enables the transfer of statistical approaches from one field to the other. For instance, we introduce intrinsic logistic-normal graphical models for compositional data, which are based on H\"usler-Reiss graphical models for extremes. Conversely, we explore how dimensionality reduction methods from compositional data analysis can be applied to the analysis of multivariate extremes.

==> tikz/commutesUVpsd.tex <==
% Written by hand
\begin{tikzpicture}[x=3cm,y=2cm]

\node (SW1) at (3, 0) {$\setpsd{W}$};
\node (SU1) at (2,0) {$\setpsd{U}$};
\node (SV1) at (1,0) {$\setpsd{V}$};
\node (SUt1) at (0,0) {$\setpsdt{U}$};

\node (SW2) at (3,-1) {$\setpsd{W}$};
\node (SU2) at (2,-1) {$\setpsd{U}$};
\node (SV2) at (1,-1) {$\setpsd{V}$};
\node (SUt2) at (0,-1) {$\setpsdt{U}$};


%% This defines `\ifuseXdiagrams', unless it's defined already:
\providesetbool{useXdiagrams}{true}
%% If used in a different document, use:
% \newif\ifuseXdiagrams\useXdiagramstrue

\ifuseXdiagrams % Replace projetions P_UX with unlabelled arrows and add legend
    % Legend:
    \node at (3.5, 0) {with};
    \node (X) at (4, 0) {$\setpsd{S}$};
    \node (X1) at (4.3, 0) {};
    \node (X2) at (4.5, 0) {};
    \path
        (X2) edge [dotted, ->] node [above, xshift=0.25cm] {$\pXY{U}{\ocompl{S}}$} (X)
        (X1) edge [->] (X)
    ;

    \path[arrows=->,auto=left]
    (SU1) edge [<->] (SV1)
    (SU1) edge [<->] (SW1)
    (SUt1) edge [->] (SV1)
    (SV1) edge [bend left=15, <->] (SW1)
    (SUt1) edge [bend left=15, ->] (SU1)
    (SUt1) edge [bend left=15, ->] (SW1)
    ;
\else % Label each projection P_UX explicitly
    \path[arrows={->[harpoon]},auto=left]
    % Projections
    (SU1) edge node {$\pXY{U}{\ocompl{V}}$} (SV1)
    (SU1) edge node {$\pXY{U}{\ocompl{W}}$} (SW1)
    (SV1) edge node {$\pXY{U}{\ocompl{U}}$} (SU1)
    (SW1) edge [bend right] node {$\pXY{U}{\ocompl{V}}$} (SV1)
    (SV1) edge [bend left] node {$\pXY{U}{\ocompl{W}}$} (SW1)
    (SW1) edge node {$\pXY{U}{\ocompl{U}}$} (SU1)
    (SUt1) edge [->] node {$\pXY{U}{\ocompl{V}}$} (SV1)
    ;
\fi


\path[arrows={->[harpoon]},auto=left]

% MP inverses
(SU1) edge [<->] node {$\cdot\pinv$} (SU2)
(SV1) edge [<->] node {$\cdot\pinv$} (SV2)
(SW1) edge [<->] node {$\cdot\pinv$} (SW2)
(SUt1) edge [<->] node {$\cdot\pinv$} (SUt2)

% Projections applied to MP inverses
(SU2) edge node {$\pXY{V}{\ocompl{V}}$} (SV2)
(SU2) edge node {$\pXY{W}{\ocompl{W}}$} (SW2)

(SV2) edge node {$\pXY{V}{\ocompl{U}}$} (SU2)
(SW2) edge node {$\pXY{W}{\ocompl{U}}$} (SU2)


;
\end{tikzpicture}



==> tikz/commutesVOnevecGammaWithW.tex <==
% Written by hand
\begin{tikzpicture}[x=3cm,y=3cm]

\node (DOne) at (1.5, 0) {$\setcnd$};

\node (Sv) at (3, -1) {$\setpsd{v}$};
\node (SOne) at (2, -1) {$\setpsd{\onevec}$};
\node (Sw) at (1, -1) {$\setpsd{w}$};
\node (S) at (0, -1) {$\setpsdt{\onevec}$};

\node (Sv2) at (3, -2) {$\setpsd{v}$};
\node (SOne2) at (2,-2) {$\setpsd{\onevec}$};
\node (Sw2) at (1, -2) {$\setpsd{w}$};
\node (S2) at (0, -2) {$\setpsdt{\onevec}$};

% Labels
\node at (-0.5, 0) {$\boxed{\Gamma}$};
\node at (-0.5, -1) {$\boxed{\Sigma}$};
\node at (-0.5, -2) {$\boxed{\Theta}$};

\path[arrows={->[harpoon]},auto=left]

% variogram inverses
(DOne) edge [bend left = 10] node [xshift=-0.2cm] {$-\half\pxyo{\onevec}{\onevec}$} (SOne)
(DOne) edge [bend left = 30] node [right] {$-\half\pxyo{\onevec}{v}$} (Sv)
(DOne) edge [bend right = 10] node [right, xshift=-0.1cm] {$-\half\pxyo{\onevec}{w}$} (Sw)

% variogram maps
(Sv) edge [bend right = 30] node [below, yshift=-0.5cm, xshift=0.5cm] {$\vario$} (DOne)
(Sw) edge [bend left = 10] node [left] {$\vario$} (DOne)
(SOne) edge [bend right = 10] node [yshift=-0.4cm, xshift=0.2cm] {$\vario$} (DOne)
(S) edge [bend left = 30, ->] node {$\vario$} (DOne)

% Projections
% Sigma row, neighbours
(Sv) edge node {$\pxyo{\onevec}{\onevec}$} (SOne)
(SOne) edge node {$\pxyo{\onevec}{v}$} (Sv)
(Sw) edge node  {$\pxyo{\onevec}{\onevec}$} (SOne)
(SOne) edge node  {$\pxyo{\onevec}{w}$} (Sw)
(S) edge [->] node [above] {$\pxyo{\onevec}{w}$} (Sw)
% Sigma row, non-neighbours
(S) edge [bend right=20, ->, gray] node [below, xshift=-1.5cm, yshift=0.2cm]{} (Sv)
(S) edge [bend right=20, ->, gray] node [below, xshift=-1.5cm, yshift=0.2cm]{} (SOne)
(Sw) edge [bend right=20, <->, gray] node [below, xshift=-1.5cm, yshift=0.2cm]{} (Sv)

% Theta row
(Sv2) edge node {$\pxyo{v}{\onevec}$} (SOne2)
(SOne2) edge node {$\pxyo{v}{v}$} (Sv2)
(Sw2) edge node {$\pxyo{w}{\onevec}$} (SOne2)
(SOne2) edge node {$\pxyo{w}{w}$} (Sw2)

% MP inverses
(Sv) edge [<->] node {$\cdot\pinv$} (Sv2)
(Sw) edge [<->] node {$\cdot\pinv$} (Sw2)
(SOne2) edge [<->] node {$\cdot\pinv$} (SOne)

% Actual inverse
(S2) edge [<->] node {$\cdot\pinv$} (S)



;
\end{tikzpicture}



==> tikz/commutesVectors.tex <==
% Written by hand
\begin{tikzpicture}[x=3cm,y=2cm]

\node (W) at (3,0) {$\ocompl{W}$};
\node (U) at (2,0) {$\ocompl{U}$};
\node (V) at (1,0) {$\ocompl{V}$};
\node (Rd) at (0,0) {$\Rd$};

%% This defines `\ifuseXdiagrams', unless it's defined already:
\providesetbool{useXdiagrams}{true}
%% If used in a different document, use:
% \newif\ifuseXdiagrams\useXdiagramstrue

\ifuseXdiagrams % Replace projetions P_UX with unlabelled arrows and add legend
    % Legend:
    \node at (3.5, 0) {with};
    \node (X) at (4, 0) {$\ocompl{S}$};
    \node (X1) at (4.3, 0) {};
    \node (X2) at (4.5, 0) {};
    \path
        (X2) edge [dotted, ->] node [above, xshift=0.25cm] {$\PXY{U}{\ocompl{S}}$} (X)
        (X1) edge [->] (X)
    ;

    \path[arrows=->,auto=left]
    (U) edge [<->] (V)
    (U) edge [<->] (W)
    (Rd) edge [->] (V)
    (V) edge [bend left=15, <->] (W)
    (Rd) edge [bend left=15, ->] (U)
    (Rd) edge [bend left=15, ->] (W)
    ;
\else % Label each projection P_UX explicitly
    \path[arrows={->[harpoon]},auto=left]

    % Straight arrows
    (U) edge node {$\PXY{U}{\ocompl{V}}$} (V)
    (V) edge node {$\PXY{U}{\ocompl{U}}$} (U)
    (U) edge node {$\PXY{U}{\ocompl{W}}$} (W)
    (W) edge node {$\PXY{U}{\ocompl{U}}$} (U)

    (Rd) edge [->] node {$\PXY{U}{\ocompl{V}}$} (V)

    % Curved arrows
    (V) edge [bend left] node {$\PXY{U}{\ocompl{W}}$} (W)
    (W) edge [bend right] node {$\PXY{U}{\ocompl{V}}$} (V)

    ;
\fi

\end{tikzpicture}


==> tikz/commutesX.tex <==
% Written by hand
\begin{tikzpicture}[x=3cm,y=2cm]

% Im X spaces
\node (MW) at (3,0) {$\setMv{W}$};
\node (MU) at (2,0) {$\setMv{U}$};
\node (MV) at (1,0) {$\setMv{V}$};
\node (MUt) at (0,0) {$\setMvt{U}$};

% ker X spaces
\node (LW) at (3,-1) {$\setMv{W}\T$};
\node (LU) at (2,-1) {$\setMv{U}\T$};
\node (LV) at (1,-1) {$\setMv{V}\T$};
\node (LUt) at (0,-1) {$(\setMvt{U})\T$};

% Im X spaces (transpose)
\node (MW2) at (3,-2) {$\setMv{W}$};
\node (MU2) at (2,-2) {$\setMv{U}$};
\node (MV2) at (1,-2) {$\setMv{V}$};
\node (MUt2) at (0,-2) {$\setMvt{U}$};


%% This defines `ifX', unless it's defined already:
\providesetbool{useXdiagrams}{true}
%% If used in a different document, use:
% \newif\ifuseXdiagrams\useXdiagramstrue

\ifuseXdiagrams % Replace projetions P_UX with unlabelled arrows and add legend
    % Legend:
    \node at (3.5, 0) {with};
    \node (X) at (4, 0) {$\ocompl{S}$};
    \node (X1) at (4.3, 0) {};
    \node (X2) at (4.5, 0) {};
    \path
        (X2) edge [dotted, ->] node [above, xshift=0.25cm] {$\PXY{U}{\ocompl{S}}\cdot$} (X)
        (X1) edge [->] (X)
    ;

    \path[arrows={->}]
    % Left projections
    (MU) edge [<->] (MV)
    (MU) edge [<->] (MW)

    (MV) edge [bend left=15, <->] (MW)

    (MUt) edge [->] (MV)
    (MUt) edge [->, bend left=15] (MU)
    (MUt) edge [->, bend left=15] (MW)
    ;
\else % Label each projection P_UX explicitly
    \path[arrows={->[harpoon]},auto=left]

    % Left projections
    (MU) edge node {$\PXY{U}{\ocompl{V}}\cdot$} (MV)
    (MV) edge node {$\PXY{U}{\ocompl{U}}\cdot$} (MU)
    (MU) edge node {$\PXY{U}{\ocompl{W}}\cdot$} (MW)
    (MW) edge node {$\PXY{U}{\ocompl{U}}\cdot$} (MU)

    (MW) edge [bend right] node {$\PXY{U}{\ocompl{V}}\cdot$} (MV)
    (MV) edge [bend left] node {$\PXY{U}{\ocompl{W}}\cdot$} (MW)

    (MUt) edge [->] node {$\PXY{U}{\ocompl{V}}\cdot$} (MV)
    ;
\fi

\path[arrows={->[harpoon]},auto=left]

% MP inverses
(MU) edge [<->] node {$\cdot\pinv$} (LU)
(MV) edge [<->] node {$\cdot\pinv$} (LV)
(MW) edge [<->] node {$\cdot\pinv$} (LW)
(MUt) edge [<->] node {$\cdot\pinv$} (LUt)

% Right projections
(LU) edge node {$\cdot\PXY{V}{\ocompl{V}}$} (LV)
(LV) edge node {$\cdot\PXY{U}{\ocompl{V}}$} (LU)
(LU) edge node {$\cdot\PXY{W}{\ocompl{W}}$} (LW)
(LW) edge node {$\cdot\PXY{U}{\ocompl{W}}$} (LU)

% Transposes
(LU) edge [<->] node {$\cdot\T$} (MU2)
(LV) edge [<->] node {$\cdot\T$} (MV2)
(LW) edge [<->] node {$\cdot\T$} (MW2)
(LUt) edge [<->] node {$\cdot\T$} (MUt2)

% Left projections after transpose
(MU2) edge node {$\PXY{V}{\ocompl{V}}\cdot$} (MV2)
(MV2) edge node {$\PXY{V}{\ocompl{U}}\cdot$} (MU2)
(MU2) edge node {$\PXY{W}{\ocompl{W}}\cdot$} (MW2)
(MW2) edge node {$\PXY{W}{\ocompl{U}}\cdot$} (MU2)

;
\end{tikzpicture}



==> tikzR/densityProjections/OneVec.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] (  0.00,  0.00) --
	(154.86,  0.00) --
	(  0.00,154.86) --
	cycle;
\definecolor{fillColor}{RGB}{190,190,190}

\path[fill=fillColor] (  0.00,  0.00) --
	( 61.95,  0.00) --
	( 61.95, 92.92) --
	(  0.00, 92.92) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 92.92) -- (216.81, 92.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 91.11) --
	(216.81, 92.92) --
	(213.68, 94.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.75,213.68) --
	( 61.95,216.81) --
	( 60.14,213.68);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 61.95, 92.92) -- ( 77.43,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 77.28,108.25) -- ( 77.43,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 75.94,102.82) --
	( 77.43,108.41) --
	( 71.85,106.91);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 83.43,106.11) {$\mathbf{1}/2$};

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (  0.00,154.86) -- (216.81,-61.95);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 92.92) -- ( 92.92, 61.95);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 85.94, 63.82) --
	( 92.92, 61.95) --
	( 91.05, 68.93);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 92.92, 61.95) -- (185.84,154.86);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (183.97,147.88) --
	(185.84,154.86) --
	(178.86,152.99);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (185.84,154.86) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 92.92, 61.95) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 85.18, 75.69) {$W^{\mathbf{1}}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.96,124.69) {$E \cdot \mathbf{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (185.84,160.86) {$Y^{\mathbf{1}}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.07, 81.18) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95,204.60) {$\mathbb{R}$};
\end{scope}
\end{tikzpicture}


==> tikzR/densityProjections/V_onePerp.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] (  0.00,  0.00) --
	(216.81,  0.00) --
	(216.81, 15.49) --
	(  0.00,123.89) --
	cycle;
\definecolor{fillColor}{RGB}{190,190,190}

\path[fill=fillColor] (  0.00,  0.00) --
	( 61.95,  0.00) --
	( 61.95, 92.92) --
	(  0.00, 92.92) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 92.92) -- (216.81, 92.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 91.11) --
	(216.81, 92.92) --
	(213.68, 94.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.75,213.68) --
	( 61.95,216.81) --
	( 60.14,213.68);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 61.95, 92.92) -- ( 72.27,113.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.17,113.36) -- ( 72.27,113.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.62,107.80) --
	( 72.27,113.57) --
	( 67.45,110.38);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 72.27,119.57) {$v$};

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (  0.00,123.89) -- (216.81, 15.49);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (  0.00,154.86) -- (216.81,-61.95);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] ( 61.95, 92.92) -- ( 92.92,123.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 92.61,123.58) -- ( 92.92,123.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 91.42,118.31) --
	( 92.92,123.89) --
	( 87.33,122.40);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 98.92,121.60) {$\mathbf{1}$};

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (108.41, 46.46) -- (123.89, 61.95);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 92.92) -- (123.89, 61.95);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (116.68, 61.51) --
	(123.89, 61.95) --
	(119.91, 67.98);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (123.89, 61.95) -- (201.32,139.38);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (199.45,132.40) --
	(201.32,139.38) --
	(194.34,137.51);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.32,139.38) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (123.89, 61.95) circle (  2.25);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (108.41, 75.69) {$W^{v}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (184.09,113.85) {$E \cdot \mathbf{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.32,145.38) {$Y^{v}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.07, 81.18) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95,204.60) {$\mathbb{R}$};
\end{scope}
\end{tikzpicture}


==> tikzR/densityProjections/e1.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] (  0.00,  0.00) --
	( 61.95,  0.00) --
	( 61.95,216.81) --
	(  0.00,216.81) --
	cycle;
\definecolor{fillColor}{RGB}{190,190,190}

\path[fill=fillColor] (  0.00,  0.00) --
	( 61.95,  0.00) --
	( 61.95, 92.92) --
	(  0.00, 92.92) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00, 92.92) -- (216.81, 92.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68, 91.11) --
	(216.81, 92.92) --
	(213.68, 94.73);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.95,  0.00) -- ( 61.95,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.75,213.68) --
	( 61.95,216.81) --
	( 60.14,213.68);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 92.92) -- ( 61.95, 30.97);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 58.33, 37.23) --
	( 61.95, 30.97) --
	( 65.56, 37.23);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] ( 61.95, 30.97) -- (185.84,154.86);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (183.97,147.88) --
	(185.84,154.86) --
	(178.86,152.99);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (185.84,154.86) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 61.95, 30.97) circle (  2.25);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95, 59.65) {$W^{e_1}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (154.67,115.40) {$E \cdot \mathbf{1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (185.84,160.86) {$Y^{e_1}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.07, 81.18) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 67.95,204.60) {$\mathbb{R}$};
\end{scope}
\end{tikzpicture}


==> tikzR/gemas/graph_cclasso.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{169,169,169}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (194.99,110.12) -- ( 31.87,151.28);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (197.47,102.89) -- (135.15, 23.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (190.81,142.65) -- (105.87,197.96);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (189.70,139.40) -- ( 32.06,152.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (175.16,167.67) -- ( 76.79,192.49);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (176.79,161.22) -- ( 49.25, 44.21);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (177.64,160.43) -- ( 74.31, 28.12);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (183.11,159.05) -- (195.53, 84.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.90,180.22) -- (102.28, 21.65);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (123.86,198.65) -- ( 76.98,194.78);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (126.53,193.71) -- ( 29.39, 69.33);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (129.69,192.32) -- (101.16, 21.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 67.72,187.58) -- ( 27.36, 70.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.31,188.69) -- (177.64, 56.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 32.06, 63.24) -- (174.97, 51.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 50.88, 41.19) -- (189.89, 76.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (136.71, 21.40) -- (176.08, 47.04);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.78,108.40) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (196.68,138.83) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.95,165.95) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.18,186.84) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (130.84,199.23) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (100.00,201.78) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 70.00,194.21) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 44.09,177.34) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 25.08,153.00) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.03,123.83) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.03, 92.98) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 25.08, 63.81) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 44.09, 39.47) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 70.00, 22.60) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (100.00, 15.03) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (130.84, 17.58) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.18, 29.97) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.95, 50.86) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (196.68, 77.98) circle (  7.00);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,139}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.78,104.96) {Al};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (196.68,135.38) {Ba};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (181.95,162.51) {Ca};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (159.18,183.40) {Cr};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (130.84,195.79) {Fe};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (100.00,198.33) {K};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 70.00,191.73) {Mg};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 44.09,173.89) {Mn};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 25.08,149.55) {Na};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.03,120.38) {Nb};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.03, 89.54) {P};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 25.08, 60.37) {Si};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 44.09, 36.03) {Sr};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 70.00, 19.16) {Ti};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (100.00, 11.59) {V};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (130.84, 14.14) {Y};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (159.18, 26.53) {Zn};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (181.95, 47.41) {Zr};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (196.68, 74.54) {LOI};
\end{scope}
\end{tikzpicture}


==> tikzR/gemas/graph_eglearn.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{169,169,169}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (197.47,113.92) -- (135.15,193.71);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (196.62,113.14) -- (105.16,197.04);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (195.91,104.58) -- ( 75.87, 26.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (190.81,142.65) -- (105.87,197.96);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (189.70,139.40) -- ( 32.06,152.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (176.79,161.22) -- ( 49.25, 44.21);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (183.11,159.05) -- (195.53, 84.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.90,180.22) -- (102.28, 21.65);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (123.86,198.65) -- ( 76.98,194.78);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (124.05,197.52) -- ( 50.88,179.05);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (129.69,192.32) -- (101.16, 21.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (132.00,192.32) -- (158.03, 36.88);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 18.37,117.67) -- ( 66.66, 28.76);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 20.19,119.09) -- (125.68, 22.31);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 22.01, 92.41) -- (189.70, 78.56);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 32.06, 63.24) -- (174.97, 51.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 76.79, 20.89) -- ( 93.21, 16.75);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.78,108.40) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (196.68,138.83) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.95,165.95) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.18,186.84) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (130.84,199.23) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (100.00,201.78) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 70.00,194.21) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 44.09,177.34) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 25.08,153.00) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.03,123.83) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.03, 92.98) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 25.08, 63.81) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 44.09, 39.47) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 70.00, 22.60) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (100.00, 15.03) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (130.84, 17.58) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (159.18, 29.97) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.95, 50.86) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (196.68, 77.98) circle (  7.00);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,139}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.78,104.96) {Al};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (196.68,135.38) {Ba};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (181.95,162.51) {Ca};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (159.18,183.40) {Cr};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (130.84,195.79) {Fe};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (100.00,198.33) {K};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 70.00,191.73) {Mg};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 44.09,173.89) {Mn};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 25.08,149.55) {Na};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.03,120.38) {Nb};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.03, 89.54) {P};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 25.08, 60.37) {Si};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 44.09, 36.03) {Sr};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 70.00, 19.16) {Ti};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (100.00, 11.59) {V};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (130.84, 14.14) {Y};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (159.18, 26.53) {Zn};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (181.95, 47.41) {Zr};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (196.68, 74.54) {LOI};
\end{scope}
\end{tikzpicture}


==> tikzR/logistic_gauss/graph_base.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{169,169,169}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 96.06,201.01) -- ( 57.59,201.66);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (103.39,193.89) -- (106.39,129.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.29,194.46) -- ( 64.86,112.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 96.73,197.91) -- ( 21.37,162.53);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 54.64,196.06) -- (102.66,128.29);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.42,194.82) -- ( 61.25,112.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 46.08,196.42) -- ( 19.54,164.91);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.15,120.13) -- ( 68.65,108.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.22,125.19) -- ( 21.53,156.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (110.98,117.02) -- (137.46, 82.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (109.38,116.10) -- (139.68, 42.70);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.74,116.80) -- ( 54.81, 47.07);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (105.65,115.65) -- ( 91.22, 21.95);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (113.67,121.80) -- (194.82,112.72);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 57.46,111.25) -- ( 19.65,154.29);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 68.66,103.59) -- (135.14, 79.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 67.37,101.39) -- (137.07, 40.82);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 60.88, 99.09) -- ( 52.05, 48.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 64.15, 99.30) -- ( 88.09, 21.72);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (141.83, 69.98) -- (142.25, 43.23);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.21, 74.42) -- ( 57.37, 43.86);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (137.24, 71.60) -- ( 94.64, 20.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (147.78, 80.51) -- (195.72,108.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.36, 36.62) -- ( 57.84, 40.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.87, 33.59) -- ( 96.64, 17.67);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (146.68, 41.74) -- (197.45,106.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 56.67, 37.41) -- ( 84.33, 18.92);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (103.06,200.89) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 50.59,201.78) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (106.71,122.57) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 62.08,105.99) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.03,159.55) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (141.72, 76.98) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (142.35, 36.23) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 50.85, 41.30) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 90.15, 15.03) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.78,111.94) circle (  7.00);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,139}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (103.06,197.68) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.59,198.57) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (106.71,119.37) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 62.08,102.78) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.03,156.34) {5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (141.72, 73.78) {6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (142.35, 33.02) {7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.85, 38.10) {8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 90.15, 11.83) {9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.78,108.73) {10};
\end{scope}
\end{tikzpicture}


==> tikzR/logistic_gauss/graph_eglearn.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{169,169,169}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 96.06,201.01) -- ( 57.59,201.66);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (103.39,193.89) -- (106.39,129.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.29,194.46) -- ( 64.86,112.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 96.73,197.91) -- ( 21.37,162.53);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.58,193.90) -- ( 90.64, 22.02);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 54.64,196.06) -- (102.66,128.29);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.42,194.82) -- ( 61.25,112.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 46.08,196.42) -- ( 19.54,164.91);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.15,120.13) -- ( 68.65,108.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.22,125.19) -- ( 21.53,156.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (110.98,117.02) -- (137.46, 82.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (109.38,116.10) -- (139.68, 42.70);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (113.67,121.80) -- (194.82,112.72);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 57.46,111.25) -- ( 19.65,154.29);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 68.66,103.59) -- (135.14, 79.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 67.37,101.39) -- (137.07, 40.82);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 60.88, 99.09) -- ( 52.05, 48.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 64.15, 99.30) -- ( 88.09, 21.72);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (141.83, 69.98) -- (142.25, 43.23);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.21, 74.42) -- ( 57.37, 43.86);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (137.24, 71.60) -- ( 94.64, 20.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (147.78, 80.51) -- (195.72,108.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.36, 36.62) -- ( 57.84, 40.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.87, 33.59) -- ( 96.64, 17.67);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (146.68, 41.74) -- (197.45,106.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 56.67, 37.41) -- ( 84.33, 18.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 95.44, 19.62) -- (196.49,107.35);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{230,159,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (103.06,200.89) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 50.59,201.78) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (106.71,122.57) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 62.08,105.99) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.03,159.55) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (141.72, 76.98) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (142.35, 36.23) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 50.85, 41.30) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 90.15, 15.03) circle (  7.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.78,111.94) circle (  7.00);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,139}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (103.06,197.68) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.59,198.57) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (106.71,119.37) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 62.08,102.78) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.03,156.34) {5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (141.72, 73.78) {6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (142.35, 33.02) {7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.85, 38.10) {8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 90.15, 11.83) {9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.78,108.73) {10};
\end{scope}
\end{tikzpicture}


==> tikzR/lr_selection/danube_aclust_dendrogram.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 32.79, 20.50) {V23};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 38.74, 20.50) {V24};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 31.14, 27.16) --
	( 31.14, 43.67) --
	( 37.09, 43.67) --
	( 37.09, 27.16);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 44.70, 22.61) {V27};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 50.65, 20.79) {V25};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 56.60, 20.79) {V26};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 48.99, 27.45) --
	( 48.99, 43.96) --
	( 54.94, 43.96) --
	( 54.94, 27.45);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 43.04, 29.27) --
	( 43.04, 45.79) --
	( 51.97, 45.79) --
	( 51.97, 43.96);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 34.12, 43.67) --
	( 34.12, 71.85) --
	( 47.51, 71.85) --
	( 47.51, 45.79);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 62.55, 21.79) {V28};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 68.50, 21.79) {V29};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 60.90, 28.45) --
	( 60.90, 44.97) --
	( 66.85, 44.97) --
	( 66.85, 28.45);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 74.45, 21.57) {V1};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 80.40, 21.57) {V13};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.80, 28.24) --
	( 72.80, 44.75) --
	( 78.75, 44.75) --
	( 78.75, 28.24);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 86.35, 22.02) {V30};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 92.30, 22.02) {V31};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 84.70, 28.68) --
	( 84.70, 45.19) --
	( 90.65, 45.19) --
	( 90.65, 28.68);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 75.77, 44.75) --
	( 75.77, 50.36) --
	( 87.67, 50.36) --
	( 87.67, 45.19);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 63.87, 44.97) --
	( 63.87, 57.92) --
	( 81.72, 57.92) --
	( 81.72, 50.36);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 98.25, 22.31) {V17};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (104.21, 20.56) {V18};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (110.16, 20.56) {V19};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.55, 27.22) --
	(102.55, 43.73) --
	(108.50, 43.73) --
	(108.50, 27.22);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 96.60, 28.98) --
	( 96.60, 45.49) --
	(105.53, 45.49) --
	(105.53, 43.73);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (116.11, 22.94) {V16};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (122.06, 20.69) {V14};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (128.01, 20.69) {V15};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (120.40, 27.36) --
	(120.40, 43.87) --
	(126.36, 43.87) --
	(126.36, 27.36);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (114.45, 29.60) --
	(114.45, 46.12) --
	(123.38, 46.12) --
	(123.38, 43.87);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (101.06, 45.49) --
	(101.06, 52.19) --
	(118.92, 52.19) --
	(118.92, 46.12);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (133.96, 23.38) {V10};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (139.91, 20.91) {V8};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (145.86, 20.91) {V9};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (138.26, 27.57) --
	(138.26, 44.08) --
	(144.21, 44.08) --
	(144.21, 27.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (132.31, 30.05) --
	(132.31, 46.56) --
	(141.23, 46.56) --
	(141.23, 44.08);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (151.81, 21.03) {V5};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (157.76, 20.52) {V6};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (163.71, 20.52) {V7};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.11, 27.18) --
	(156.11, 43.69) --
	(162.06, 43.69) --
	(162.06, 27.18);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (150.16, 27.70) --
	(150.16, 44.21) --
	(159.09, 44.21) --
	(159.09, 43.69);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (169.67, 21.20) {V2};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (175.62, 20.61) {V3};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (181.57, 20.61) {V4};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (173.96, 27.28) --
	(173.96, 43.79) --
	(179.91, 43.79) --
	(179.91, 27.28);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (168.01, 27.86) --
	(168.01, 44.37) --
	(176.94, 44.37) --
	(176.94, 43.79);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (154.62, 44.21) --
	(154.62, 48.08) --
	(172.48, 48.08) --
	(172.48, 44.37);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (136.77, 46.56) --
	(136.77, 54.58) --
	(163.55, 54.58) --
	(163.55, 48.08);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (187.52, 24.03) {V22};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (193.47, 21.37) {V20};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (199.42, 21.37) {V21};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (191.82, 28.04) --
	(191.82, 44.55) --
	(197.77, 44.55) --
	(197.77, 28.04);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (185.87, 30.69) --
	(185.87, 47.20) --
	(194.79, 47.20) --
	(194.79, 44.55);

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (205.37, 25.91) {V11};

\node[text=drawColor,rotate= 90.00,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.80] at (211.32, 25.91) {V12};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (203.72, 32.58) --
	(203.72, 49.09) --
	(209.67, 49.09) --
	(209.67, 32.58);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (190.33, 47.20) --
	(190.33, 64.10) --
	(206.69, 64.10) --
	(206.69, 49.09);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (150.16, 54.58) --
	(150.16, 81.27) --
	(198.51, 81.27) --
	(198.51, 64.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (109.99, 52.19) --
	(109.99,101.42) --
	(174.34,101.42) --
	(174.34, 81.27);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.80, 57.92) --
	( 72.80,154.15) --
	(142.16,154.15) --
	(142.16,101.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.81, 71.85) --
	( 40.81,208.78) --
	(107.48,208.78) --
	(107.48,154.15);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00, 43.66) -- ( 24.00,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00, 43.66) -- ( 18.00, 43.66);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00, 90.07) -- ( 18.00, 90.07);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00,136.48) -- ( 18.00,136.48);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00,182.89) -- ( 18.00,182.89);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (  9.60, 43.66) {0.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (  9.60, 90.07) {0.2};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (  9.60,136.48) {0.4};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (  9.60,182.89) {0.6};
\end{scope}
\end{tikzpicture}


==> tikzR/lr_selection/danube_step_graph.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (252.94,252.94);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (252.94,252.94);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 6.0pt,line join=round,line cap=round] (124.90,235.65) -- (157.65,225.42);

\path[draw=drawColor,line width= 5.8pt,line join=round,line cap=round] (154.20, 45.81) -- (172.74, 54.51);

\path[draw=drawColor,line width= 5.6pt,line join=round,line cap=round] ( 95.00,110.01) -- (113.54,101.31);

\path[draw=drawColor,line width= 5.4pt,line join=round,line cap=round] ( 69.15,221.01) -- ( 50.60,212.31);

\path[draw=drawColor,line width= 5.2pt,line join=round,line cap=round] (163.47,174.20) -- (163.47,175.87);

\path[draw=drawColor,line width= 5.0pt,line join=round,line cap=round] (163.47,201.95) -- (163.47,203.62);

\path[draw=drawColor,line width= 4.8pt,line join=round,line cap=round] ( 80.50,225.42) -- (113.25,235.65);

\path[draw=drawColor,line width= 4.6pt,line join=round,line cap=round] ( 80.20,221.01) -- ( 98.74,212.31);

\path[draw=drawColor,line width= 4.4pt,line join=round,line cap=round] (163.47,189.74) -- (163.47,188.08);

\path[draw=drawColor,line width= 4.2pt,line join=round,line cap=round] (178.27, 78.74) -- (178.27, 77.08);

\path[draw=drawColor,line width= 4.0pt,line join=round,line cap=round] (178.27, 64.87) -- (178.27, 63.20);

\path[draw=drawColor,line width= 3.8pt,line join=round,line cap=round] (172.74, 26.76) -- (154.20, 18.06);

\path[draw=drawColor,line width= 3.6pt,line join=round,line cap=round] (163.47,215.83) -- (163.47,217.49);

\path[draw=drawColor,line width= 3.4pt,line join=round,line cap=round] (202.34, 45.81) -- (183.80, 54.51);

\path[draw=drawColor,line width= 3.2pt,line join=round,line cap=round] (139.40,142.94) -- (157.94,151.63);

\path[draw=drawColor,line width= 3.0pt,line join=round,line cap=round] (178.27,104.83) -- (178.27,106.49);

\path[draw=drawColor,line width= 2.8pt,line join=round,line cap=round] (183.80, 26.76) -- (202.34, 18.06);

\path[draw=drawColor,line width= 2.6pt,line join=round,line cap=round] (187.54,142.94) -- (169.00,151.63);

\path[draw=drawColor,line width= 2.4pt,line join=round,line cap=round] (119.07, 90.95) -- (119.07, 92.62);

\path[draw=drawColor,line width= 2.2pt,line join=round,line cap=round] (183.80, 31.94) -- (202.34, 40.63);

\path[draw=drawColor,line width= 2.0pt,line join=round,line cap=round] ( 69.15,198.44) -- ( 50.60,207.13);

\path[draw=drawColor,line width= 1.8pt,line join=round,line cap=round] (178.27, 92.62) -- (178.27, 90.95);

\path[draw=drawColor,line width= 1.6pt,line join=round,line cap=round] (119.07, 78.74) -- (119.07, 77.08);

\path[draw=drawColor,line width= 1.4pt,line join=round,line cap=round] ( 65.40,101.31) -- ( 83.94,110.01);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (133.87,132.58) -- (133.87,134.24);

\path[draw=drawColor,line width= 1.0pt,line join=round,line cap=round] (128.05,124.65) -- ( 95.30,114.42);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 21.00,198.44) -- ( 39.55,207.13);

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] (139.70,124.65) -- (172.45,114.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (163.47,161.99) -- (163.47,160.33);

\path[draw=drawColor,line width= 0.2pt,line join=round,line cap=round] (231.94, 31.94) -- (213.40, 40.63);
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.47,195.85) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (133.87,126.47) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (133.87,140.35) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (148.67, 43.22) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 15.47,195.85) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (178.27, 29.35) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 59.87, 98.72) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 74.67,223.60) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 89.47,112.60) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (178.27, 98.72) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (178.27, 84.85) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.47,168.10) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (119.07, 84.85) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.47,181.97) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (148.67, 15.47) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (119.07, 98.72) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (193.07,140.35) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.47,209.72) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.47,154.22) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (119.07,237.47) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 74.67,195.85) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (178.27, 70.97) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (237.47, 29.35) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 45.07,209.72) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (207.87, 43.22) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (119.07, 70.97) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (163.47,223.60) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (104.27,209.72) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (178.27,112.60) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (207.87, 15.47) circle (  6.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (178.27, 57.10) circle (  6.10);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (252.94,252.94);
\definecolor{drawColor}{RGB}{0,0,139}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.47,192.64) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (133.87,123.26) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (133.87,137.14) {3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (148.67, 40.02) {4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 15.47,192.64) {5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (178.27, 26.14) {6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 59.87, 95.52) {7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 74.67,220.39) {8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 89.47,109.39) {9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (178.27, 95.52) {10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (178.27, 81.64) {11};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.47,164.89) {12};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (119.07, 81.64) {13};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.47,178.76) {14};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (148.67, 12.27) {15};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (119.07, 95.52) {16};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (193.07,137.14) {17};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.47,206.51) {18};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.47,151.01) {19};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (119.07,234.26) {20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 74.67,192.64) {21};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (178.27, 67.77) {22};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (237.47, 26.14) {23};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 45.07,206.51) {24};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (207.87, 40.02) {25};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (119.07, 67.77) {26};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (163.47,220.39) {27};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (104.27,206.51) {28};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (178.27,109.39) {29};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (207.87, 12.27) {30};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (178.27, 53.89) {31};
\end{scope}
\end{tikzpicture}


==> tikzR/lra/lra_unweighted.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (325.21,325.21);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,325.21);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 73.38, 61.20) -- (265.10, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 73.38, 61.20) -- ( 73.38, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (137.29, 61.20) -- (137.29, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (201.19, 61.20) -- (201.19, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (265.10, 61.20) -- (265.10, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 73.38, 39.60) {-2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (137.29, 39.60) {-1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.19, 39.60) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (265.10, 39.60) {1};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 92.03) -- ( 49.20,251.79);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 92.03) -- ( 43.20, 92.03);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,123.98) -- ( 43.20,123.98);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,155.93) -- ( 43.20,155.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,187.89) -- ( 43.20,187.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,219.84) -- ( 43.20,219.84);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,251.79) -- ( 43.20,251.79);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 92.03) {-1.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,123.98) {-1.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,155.93) {-0.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,187.89) {0.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,219.84) {0.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,251.79) {1.0};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(300.01, 61.20) --
	(300.01,276.01) --
	( 49.20,276.01) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,325.21);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (174.61, 15.60) {LRA dimension 1 (34.9{\%})};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80,168.61) {LRA dimension 2 (33.3{\%})};
\end{scope}
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (300.01,276.01);
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 49.20,187.89) -- (300.01,187.89);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (201.19, 61.20) -- (201.19,276.01);
\definecolor{drawColor}{RGB}{247,225,185}

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (219.54,138.22);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (215.90,144.47) --
	(219.54,138.22) --
	(218.25,145.34);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (170.56,218.19);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (176.50,214.08) --
	(170.56,218.19) --
	(174.74,212.29);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (159.44,222.68);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.72,219.08) --
	(159.44,222.68) --
	(164.11,217.16);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (154.87,227.11);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (161.11,223.47) --
	(154.87,227.11) --
	(159.49,221.55);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (191.28,252.64);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (193.59,245.79) --
	(191.28,252.64) --
	(191.11,245.41);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (202.68,252.55);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (203.77,245.41) --
	(202.68,252.55) --
	(201.27,245.46);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (202.04,252.85);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (203.20,245.72) --
	(202.04,252.85) --
	(200.69,245.75);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (176.42,258.87);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (179.95,252.56) --
	(176.42,258.87) --
	(177.58,251.73);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (186.51,256.98);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (189.22,250.27) --
	(186.51,256.98) --
	(186.76,249.75);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (206.18,260.42);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (206.95,253.24) --
	(206.18,260.42) --
	(204.44,253.41);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (235.69,233.06);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (232.37,226.64) --
	(235.69,233.06) --
	(230.38,228.16);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (228.66,236.85);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (226.27,230.03) --
	(228.66,236.85) --
	(224.08,231.26);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (251.63,114.95);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (246.55,120.09) --
	(251.63,114.95) --
	(248.61,121.51);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (215.79,203.26);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (211.80,197.23) --
	(215.79,203.26) --
	(209.98,198.96);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (220.77,203.34);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (215.96,197.94) --
	(220.77,203.34) --
	(214.40,199.91);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (253.53,206.83);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (247.26,203.23) --
	(253.53,206.83) --
	(246.41,205.59);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (242.49,193.95);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (235.63,191.67) --
	(242.49,193.95) --
	(235.27,194.15);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (251.37,189.26);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (244.29,187.82) --
	(251.37,189.26) --
	(244.22,190.32);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (254.49,193.04);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (247.53,191.10) --
	(254.49,193.04) --
	(247.29,193.60);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (234.76,243.33);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (232.15,236.59) --
	(234.76,243.33) --
	(230.00,237.89);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (242.27,232.08);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (238.34,226.01) --
	(242.27,232.08) --
	(236.50,227.72);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (245.55,215.83);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (240.20,210.98) --
	(245.55,215.83) --
	(238.86,213.10);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- ( 79.97,184.48);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 87.05,185.94) --
	( 79.97,184.48) --
	( 87.12,183.43);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- ( 77.55,182.53);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 84.61,184.09) --
	( 77.55,182.53) --
	( 84.72,181.58);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- ( 85.62,109.67);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 90.81,114.70) --
	( 85.62,109.67) --
	( 92.22,112.62);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- ( 79.48,111.60);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 84.84,116.44) --
	( 79.48,111.60) --
	( 86.17,114.31);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- ( 92.36, 92.83);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] ( 96.90, 98.45) --
	( 92.36, 92.83) --
	( 98.55, 96.56);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (266.79, 80.46);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (262.01, 85.88) --
	(266.79, 80.46) --
	(264.15, 87.19);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (260.41, 82.61);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (255.82, 88.20) --
	(260.41, 82.61) --
	(258.01, 89.43);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (271.55, 85.77);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (266.48, 90.92) --
	(271.55, 85.77) --
	(268.55, 92.34);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.19,187.89) -- (276.73, 88.28);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (271.43, 93.19) --
	(276.73, 88.28) --
	(273.43, 94.71);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (182.66,216.47) {\bfseries 1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (156.28,196.02) {\bfseries 2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (201.88,179.79) {\bfseries 3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (161.34,144.89) {\bfseries 4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (209.25,181.97) {\bfseries 5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (209.43,181.79) {\bfseries 6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (169.16,170.68) {\bfseries 7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (257.03,202.60) {\bfseries 8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (192.26,194.95) {\bfseries 9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (192.70,151.57) {\bfseries 10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (171.91,215.43) {\bfseries 11};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (229.78,179.80) {\bfseries 12};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (227.81,200.22) {\bfseries 13};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (247.12,134.84) {\bfseries 14};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (131.28,219.55) {\bfseries 15};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (216.50,211.84) {\bfseries 16};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (132.15,149.70) {\bfseries 17};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (182.63,169.25) {\bfseries 18};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (152.95,191.07) {\bfseries 19};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (199.12,154.52) {\bfseries 20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (220.24,187.42) {\bfseries 21};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (251.63,146.68) {\bfseries 22};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (190.53,186.27) {\bfseries 23};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (207.06, 99.24) {\bfseries 24};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (197.69,215.81) {\bfseries 25};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (183.85,200.20) {\bfseries 26};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (238.56,207.79) {\bfseries 27};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (179.60,211.70) {\bfseries 28};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (189.41,183.22) {\bfseries 29};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (257.96,193.68) {\bfseries 30};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (224.93,171.39) {\bfseries 31};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (224.02,244.43) {\bfseries 32};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (231.41,182.55) {\bfseries 33};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (176.52,153.39) {\bfseries 34};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (238.11,256.14) {\bfseries 35};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (222.26,169.36) {\bfseries 36};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (213.58,151.21) {\bfseries 37};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (174.70,233.70) {\bfseries 38};
\definecolor{drawColor}{RGB}{255,165,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (220.50,132.85) {\bfseries\itshape V1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (168.95,217.03) {\bfseries\itshape V2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (157.25,221.75) {\bfseries\itshape V3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (152.43,227.19) {\bfseries\itshape V4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (190.75,253.29) {\bfseries\itshape V5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (202.76,253.19) {\bfseries\itshape V6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (202.08,253.51) {\bfseries\itshape V7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (175.12,259.84) {\bfseries\itshape V8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (185.74,257.85) {\bfseries\itshape V9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (206.45,261.48) {\bfseries\itshape V10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (237.51,232.67) {\bfseries\itshape V11};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (230.11,236.67) {\bfseries\itshape V12};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (254.28,108.35) {\bfseries\itshape V13};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (216.56,202.08) {\bfseries\itshape V14};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (221.80,201.39) {\bfseries\itshape V15};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (256.28,205.07) {\bfseries\itshape V16};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (244.67,191.50) {\bfseries\itshape V17};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (254.01,186.58) {\bfseries\itshape V18};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (257.30,190.55) {\bfseries\itshape V19};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (236.53,243.49) {\bfseries\itshape V20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (244.43,231.64) {\bfseries\itshape V21};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (247.88,214.54) {\bfseries\itshape V22};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 73.59,181.54) {\bfseries\itshape V23};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 71.04,180.26) {\bfseries\itshape V24};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 79.54,102.79) {\bfseries\itshape V25};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 73.07,104.82) {\bfseries\itshape V26};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 86.63, 85.06) {\bfseries\itshape V27};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (270.24, 72.05) {\bfseries\itshape V28};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (263.52, 74.31) {\bfseries\itshape V29};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (275.26, 77.64) {\bfseries\itshape V30};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (280.70, 80.27) {\bfseries\itshape V31};
\end{scope}
\end{tikzpicture}


==> tikzR/lra/lra_weighted.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (325.21,325.21);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,325.21);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(300.01, 61.20) --
	(300.01,276.01) --
	( 49.20,276.01) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,325.21);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (174.61, 15.60) {LRA dimension 1 (62.9{\%})};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80,168.61) {LRA dimension 2 (13{\%})};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (325.21,325.21);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.11, 61.20) -- (291.66, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.11, 61.20) -- (102.11, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (165.30, 61.20) -- (165.30, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (228.48, 61.20) -- (228.48, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (291.66, 61.20) -- (291.66, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (102.11, 39.60) {-1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (165.30, 39.60) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (228.48, 39.60) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (291.66, 39.60) {2};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 79.22) -- ( 49.20,268.77);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 79.22) -- ( 43.20, 79.22);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,110.81) -- ( 43.20,110.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,142.40) -- ( 43.20,142.40);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,173.99) -- ( 43.20,173.99);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,205.59) -- ( 43.20,205.59);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,237.18) -- ( 43.20,237.18);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,268.77) -- ( 43.20,268.77);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 79.22) {-2.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,110.81) {-1.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,142.40) {-1.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,173.99) {-0.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,205.59) {0.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,237.18) {0.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,268.77) {1.0};
\end{scope}
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (300.01,276.01);
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 49.20,205.59) -- (300.01,205.59);

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] (165.30, 61.20) -- (165.30,276.01);
\definecolor{drawColor}{RGB}{247,225,185}

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (183.74,181.95);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (178.37,186.79) --
	(183.74,181.95) --
	(180.35,188.34);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (140.89,179.72);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (144.86,185.76) --
	(140.89,179.72) --
	(146.69,184.04);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (136.55,176.87);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (140.70,182.79) --
	(136.55,176.87) --
	(142.48,181.02);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (133.58,175.81);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (137.91,181.60) --
	(133.58,175.81) --
	(139.63,179.77);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (130.93,218.75);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (138.03,217.38) --
	(130.93,218.75) --
	(137.13,215.03);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (133.30,230.71);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (139.68,227.30) --
	(133.30,230.71) --
	(138.13,225.32);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (132.73,232.69);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (139.00,229.10) --
	(132.73,232.69) --
	(137.39,227.17);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (124.90,215.28);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (132.11,214.84) --
	(124.90,215.28) --
	(131.53,212.40);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (128.19,222.50);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (135.18,220.69) --
	(128.19,222.50) --
	(134.14,218.40);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (131.41,238.37);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (137.39,234.32) --
	(131.41,238.37) --
	(135.65,232.52);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (147.57,262.11);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (150.90,255.69) --
	(147.57,262.11) --
	(148.50,254.94);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (145.25,261.48);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (148.84,255.20) --
	(145.25,261.48) --
	(146.47,254.35);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (200.59,206.23);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (193.49,204.85) --
	(200.59,206.23) --
	(193.45,207.36);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (154.36,214.70);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (160.63,211.11) --
	(154.36,214.70) --
	(159.02,209.18);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (154.92,218.34);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (160.39,213.61) --
	(154.92,218.34) --
	(158.44,212.02);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (160.70,255.04);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (162.61,248.07) --
	(160.70,255.04) --
	(160.11,247.83);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (162.94,243.25);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (164.64,236.23) --
	(162.94,243.25) --
	(162.13,236.07);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (167.05,247.89);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (168.01,240.72) --
	(167.05,247.89) --
	(165.50,240.83);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (166.78,251.49);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (167.80,244.34) --
	(166.78,251.49) --
	(165.30,244.42);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (145.22,258.93);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (148.90,252.71) --
	(145.22,258.93) --
	(146.55,251.82);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (151.28,257.03);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (154.36,250.49) --
	(151.28,257.03) --
	(151.94,249.83);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (158.38,252.85);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (160.65,245.99) --
	(158.38,252.85) --
	(158.17,245.62);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (137.15,110.13);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (137.96,117.31) --
	(137.15,110.13) --
	(140.37,116.60);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (137.93,108.76);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (138.66,115.95) --
	(137.93,108.76) --
	(141.07,115.26);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (162.26, 83.24);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (161.18, 90.38) --
	(162.26, 83.24) --
	(163.69, 90.32);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (159.80, 82.15);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (158.86, 89.32) --
	(159.80, 82.15) --
	(161.37, 89.20);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (169.86, 86.16);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (168.33, 93.22) --
	(169.86, 86.16) --
	(170.84, 93.32);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (209.38,227.37);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (203.56,223.09) --
	(209.38,227.37) --
	(202.44,225.34);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (208.23,217.69);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (201.72,214.55) --
	(208.23,217.69) --
	(201.04,216.97);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (213.27,223.88);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (207.06,220.17) --
	(213.27,223.88) --
	(206.17,222.52);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (165.30,205.59) -- (211.87,233.13);

\path[draw=drawColor,line width= 0.8pt,line join=round,line cap=round] (206.39,228.43) --
	(211.87,233.13) --
	(205.11,230.59);
\definecolor{drawColor}{RGB}{0,0,255}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (120.06,194.28) {\bfseries 1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (128.77,176.75) {\bfseries 2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (177.45,184.21) {\bfseries 3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (180.36,184.98) {\bfseries 4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (167.86,210.26) {\bfseries 5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (179.90,204.11) {\bfseries 6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (164.13,185.55) {\bfseries 7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (182.74,227.63) {\bfseries 8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (159.67,207.19) {\bfseries 9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (195.30,193.63) {\bfseries 10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (118.69,200.98) {\bfseries 11};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (190.30,209.92) {\bfseries 12};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (164.83,222.40) {\bfseries 13};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (216.19,222.07) {\bfseries 14};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at ( 90.72,184.17) {\bfseries 15};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (136.87,209.13) {\bfseries 16};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (173.02,171.86) {\bfseries 17};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (163.18,203.58) {\bfseries 18};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (147.61,191.11) {\bfseries 19};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (202.03,184.35) {\bfseries 20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (169.71,220.15) {\bfseries 21};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (233.84,214.86) {\bfseries 22};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (149.30,202.44) {\bfseries 23};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (257.61,175.53) {\bfseries 24};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (140.24,215.59) {\bfseries 25};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (133.51,203.38) {\bfseries 26};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (156.60,226.10) {\bfseries 27};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (131.27,195.67) {\bfseries 28};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (155.05,200.19) {\bfseries 29};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (184.69,231.83) {\bfseries 30};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (196.15,205.98) {\bfseries 31};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (118.36,225.59) {\bfseries 32};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (181.21,214.33) {\bfseries 33};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (192.87,179.73) {\bfseries 34};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (131.22,222.76) {\bfseries 35};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (191.03,208.04) {\bfseries 36};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (196.78,206.79) {\bfseries 37};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (102.10,196.56) {\bfseries 38};
\definecolor{drawColor}{RGB}{255,165,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (184.71,177.95) {\bfseries\itshape V1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (139.61,175.60) {\bfseries\itshape V2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (135.04,172.60) {\bfseries\itshape V3};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (131.91,172.26) {\bfseries\itshape V4};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (129.13,216.69) {\bfseries\itshape V5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (131.62,229.27) {\bfseries\itshape V6};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (131.01,231.35) {\bfseries\itshape V7};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (122.77,213.03) {\bfseries\itshape V8};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (126.23,220.63) {\bfseries\itshape V9};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (129.62,237.33) {\bfseries\itshape V10};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (146.64,262.32) {\bfseries\itshape V11};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (144.20,261.66) {\bfseries\itshape V12};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (202.44,203.51) {\bfseries\itshape V13};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (153.78,213.20) {\bfseries\itshape V14};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (154.37,216.25) {\bfseries\itshape V15};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (160.45,254.88) {\bfseries\itshape V16};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (162.81,242.48) {\bfseries\itshape V17};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (167.14,247.35) {\bfseries\itshape V18};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (166.86,251.15) {\bfseries\itshape V19};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (144.17,258.97) {\bfseries\itshape V20};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (150.54,256.98) {\bfseries\itshape V21};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (158.01,252.58) {\bfseries\itshape V22};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (135.67,102.35) {\bfseries\itshape V23};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (136.49,101.68) {\bfseries\itshape V24};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (162.10, 74.04) {\bfseries\itshape V25};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (159.51, 72.89) {\bfseries\itshape V26};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (170.10, 77.11) {\bfseries\itshape V27};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (211.70,225.76) {\bfseries\itshape V28};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (210.49,215.57) {\bfseries\itshape V29};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (215.79,222.08) {\bfseries\itshape V30};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.80] at (214.32,231.82) {\bfseries\itshape V31};
\end{scope}
\end{tikzpicture}


==> tikzR/multivariateEVT/evtLogThresholdEx2.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] ( 24.00, 24.00) rectangle (204.81,204.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00, 40.14) -- (204.81, 40.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (201.68, 38.33) --
	(204.81, 40.14) --
	(201.68, 41.95);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.14, 24.00) -- ( 40.14,204.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 41.95,201.68) --
	( 40.14,204.81) --
	( 38.33,201.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (196.58, 28.40) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 46.14,189.34) {$\mathbb{R}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (145.21, 92.82) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 48.60,185.37) circle (  2.25);
\definecolor{drawColor}{RGB}{190,190,190}
\definecolor{fillColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 75.25, 98.66) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (106.72, 83.55) circle (  2.25);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (183.94,141.84) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (263.00,253.57) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (139.96, 72.73) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (130.64,165.16) circle (  2.25);
\definecolor{drawColor}{RGB}{190,190,190}
\definecolor{fillColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 99.07,114.94) circle (  2.25);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 59.63,156.63) circle (  2.25);
\definecolor{drawColor}{RGB}{190,190,190}
\definecolor{fillColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 64.60, 93.60) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 79.75, 61.39) circle (  2.25);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (187.42,178.95) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (241.49,162.41) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (146.88,188.15) circle (  2.25);
\definecolor{drawColor}{RGB}{190,190,190}
\definecolor{fillColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 92.66, 57.74) circle (  2.25);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (224.67,271.91) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (141.48,153.78) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (157.76,219.06) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (142.36,179.80) circle (  2.25);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (128.80, 40.14) -- (128.80, 40.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (128.80, 40.14) -- (128.80, 34.14);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (128.80, 18.54) {u};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.14,128.80) -- ( 40.14,128.80);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.14,128.80) -- ( 34.14,128.80);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 25.74,128.80) {u};
\end{scope}
\begin{scope}
\path[clip] ( 24.00, 24.00) rectangle (204.81,204.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 40.14,128.80) --
	(128.80,128.80) --
	(128.80, 40.14);
\end{scope}
\end{tikzpicture}


==> tikzR/multivariateEVT/evtLogThresholdEx3.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] ( 24.00, 24.00) rectangle (204.81,204.81);
\definecolor{fillColor}{RGB}{190,190,190}

\path[fill=fillColor] ( 24.00, 24.00) --
	(108.35, 24.00) --
	(108.35,108.35) --
	( 24.00,108.35) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00,108.35) -- (204.81,108.35);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (201.68,106.54) --
	(204.81,108.35) --
	(201.68,110.16);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (108.35, 24.00) -- (108.35,204.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (110.16,201.68) --
	(108.35,204.81) --
	(106.54,201.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (199.99, 96.61) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (114.35,194.80) {$\mathbb{R}$};
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (176.59,142.56) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (113.85,202.66) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (201.74,174.40) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (253.09,246.96) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (173.17,129.51) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (167.12,189.54) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (121.01,184.00) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (204.00,198.50) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (239.11,187.76) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (177.67,204.47) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (228.19,258.87) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.16,182.15) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (184.74,224.55) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (174.74,199.05) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (176.59,142.56) --
	(119.01, 84.99);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (113.85,202.66) --
	( 56.27,145.09);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (201.74,174.40) --
	(144.16,116.82);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (253.09,246.96) --
	(195.51,189.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (173.17,129.51) --
	(115.60, 71.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (167.12,189.54) --
	(109.54,131.96);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (121.01,184.00) --
	( 63.43,126.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (204.00,198.50) --
	(146.42,140.92);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (239.11,187.76) --
	(181.54,130.18);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (177.67,204.47) --
	(120.09,146.90);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (228.19,258.87) --
	(170.61,201.29);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (174.16,182.15) --
	(116.58,124.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (184.74,224.55) --
	(127.16,166.97);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (174.74,199.05) --
	(117.16,141.47);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (119.01, 84.99) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 56.27,145.09) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (144.16,116.82) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (195.51,189.38) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (115.60, 71.94) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (109.54,131.96) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 63.43,126.43) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (146.42,140.92) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (181.54,130.18) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (120.09,146.90) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (170.61,201.29) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (116.58,124.57) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (127.16,166.97) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (117.16,141.47) circle (  2.25);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (108.35,108.35) -- (108.35,108.35);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (108.35,108.35) -- (108.35,102.35);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (108.35,108.35) -- (108.35,108.35);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (108.35,108.35) -- (102.35,108.35);
\end{scope}
\end{tikzpicture}


==> tikzR/multivariateEVT/evtThresholdEx3.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] ( 24.00, 24.00) rectangle (204.81,204.81);
\definecolor{fillColor}{RGB}{190,190,190}

\path[fill=fillColor] ( 48.77, 48.77) --
	( 73.54, 48.77) --
	( 73.54, 73.54) --
	( 48.77, 73.54) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 24.00, 48.77) -- (204.81, 48.77);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (201.68, 46.96) --
	(204.81, 48.77) --
	(201.68, 50.58);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 48.77, 24.00) -- ( 48.77,204.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 50.58,201.68) --
	( 48.77,204.81) --
	( 46.96,201.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (197.01, 37.03) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 54.77,190.03) {$\mathbb{R}$};
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (139.84, 96.35) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 76.28,198.55) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (195.93,136.11) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (440.76,397.52) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (134.09, 85.86) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (124.79,165.37) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 80.30,153.68) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (202.41,187.10) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (349.02,161.47) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (141.73,203.81) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (292.53,486.51) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (135.72,150.04) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (155.16,276.17) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (136.68,188.57) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (139.84, 96.35) --
	( 79.12, 64.63);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 76.28,198.55) --
	( 57.94, 98.70);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (195.93,136.11) --
	( 97.82, 77.88);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (440.76,397.52) --
	(179.43,165.02);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (134.09, 85.86) --
	( 77.21, 61.13);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (124.79,165.37) --
	( 74.11, 87.63);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 80.30,153.68) --
	( 59.28, 83.74);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (202.41,187.10) --
	( 99.98, 94.88);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (349.02,161.47) --
	(148.85, 86.34);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (141.73,203.81) --
	( 79.76,100.45);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (292.53,486.51) --
	(130.02,194.68);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.72,150.04) --
	( 77.75, 82.52);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (155.16,276.17) --
	( 84.23,124.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (136.68,188.57) --
	( 78.07, 95.37);
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 79.12, 64.63) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 57.94, 98.70) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 97.82, 77.88) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (179.43,165.02) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 77.21, 61.13) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 74.11, 87.63) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 59.28, 83.74) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 99.98, 94.88) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (148.85, 86.34) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 79.76,100.45) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (130.02,194.68) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 77.75, 82.52) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 84.23,124.57) circle (  2.25);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] ( 78.07, 95.37) circle (  2.25);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 73.54, 48.77) -- ( 73.54, 48.77);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 73.54, 48.77) -- ( 73.54, 42.77);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 73.54, 27.17) {1};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 48.77, 73.54) -- ( 48.77, 73.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 48.77, 73.54) -- ( 42.77, 73.54);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.37, 73.54) {1};
\end{scope}
\begin{scope}
\path[clip] ( 24.00, 24.00) rectangle (204.81,204.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 48.77, 73.54) --
	( 73.54, 73.54) --
	( 73.54, 48.77);
\end{scope}
\end{tikzpicture}


==> tikzR/uvwProjections/proj_uv.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00,108.41) -- (216.81,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68,106.60) --
	(216.81,108.41) --
	(213.68,110.21);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 96.67) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,205.84) {$\mathbb{R}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- ( 50.59, 79.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 50.81, 79.79) -- ( 50.59, 79.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.45, 86.67) --
	( 50.59, 79.50) --
	( 57.24, 82.34);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.59, 67.76) {$u$};
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- ( 82.20,143.15);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 82.10,142.80) -- ( 82.20,143.15);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 83.95,136.14) --
	( 82.20,143.15) --
	( 77.00,138.12);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 82.20,149.15) {$v$};
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (  0.00,129.05) -- (216.81, 67.11);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (180.67,144.54) -- (139.23, 89.27);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (139.64, 89.83) -- (139.23, 89.27);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (140.09, 96.45) --
	(139.23, 89.27) --
	(145.87, 92.11);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (165.95,114.61) {$P_{uv^\perp}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (180.67,144.54) circle (  2.25);
\definecolor{drawColor}{RGB}{255,165,0}
\definecolor{fillColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (139.23, 89.27) circle (  2.25);
\end{scope}
\end{tikzpicture}


==> tikzR/uvwProjections/proj_uvwinv.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00,108.41) -- (216.81,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68,106.60) --
	(216.81,108.41) --
	(213.68,110.21);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 96.67) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,205.84) {$\mathbb{R}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- ( 50.59, 79.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 50.81, 79.79) -- ( 50.59, 79.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.45, 86.67) --
	( 50.59, 79.50) --
	( 57.24, 82.34);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.59, 67.76) {$u$};
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- ( 82.20,143.15);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 82.10,142.80) -- ( 82.20,143.15);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 83.95,136.14) --
	( 82.20,143.15) --
	( 77.00,138.12);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 82.20,149.15) {$v$};
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (  0.00,129.05) -- (216.81, 67.11);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- (104.59,124.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (104.27,124.40) -- (104.59,124.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.61,118.53) --
	(104.59,124.57) --
	( 97.38,125.00);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (104.59,130.57) {$w$};
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (  0.00,252.94) -- (216.81,-180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (180.67,144.54) -- (139.23, 89.27);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (139.64, 89.83) -- (139.23, 89.27);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (140.09, 96.45) --
	(139.23, 89.27) --
	(145.87, 92.11);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (165.95,114.61) {$P_{uv^\perp}$};

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (140.57, 88.89) -- (105.44, 42.06);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (105.44, 42.06) -- (111.82, 45.47);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (129.00, 63.18) {$P_{uw^\perp}$};

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (104.14, 44.66) -- (137.89, 89.66);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (137.89, 89.66) -- (131.51, 86.25);

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  1.00] at (115.01, 64.86) {$P_{uv^\perp}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (180.67,144.54) circle (  2.25);
\definecolor{drawColor}{RGB}{255,165,0}
\definecolor{fillColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (139.23, 89.27) circle (  2.25);
\definecolor{drawColor}{RGB}{0,0,255}
\definecolor{fillColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (104.79, 43.36) circle (  2.25);
\end{scope}
\end{tikzpicture}


==> tikzR/uvwProjections/proj_uw.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (216.81,216.81);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (216.81,216.81);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (  0.00,108.41) -- (216.81,108.41);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (213.68,106.60) --
	(216.81,108.41) --
	(213.68,110.21);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,  0.00) -- ( 72.27,216.81);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 74.08,213.68) --
	( 72.27,216.81) --
	( 70.46,213.68);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (209.58, 96.67) {$\mathbb{R}$};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 78.27,205.84) {$\mathbb{R}$};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- ( 50.59, 79.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 50.81, 79.79) -- ( 50.59, 79.50);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 51.45, 86.67) --
	( 50.59, 79.50) --
	( 57.24, 82.34);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 50.59, 67.76) {$u$};
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 72.27,108.41) -- (104.59,124.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (104.27,124.40) -- (104.59,124.57);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (100.61,118.53) --
	(104.59,124.57) --
	( 97.38,125.00);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (104.59,130.57) {$w$};
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 1pt off 3pt ,line join=round,line cap=round] (  0.00,252.94) -- (216.81,-180.67);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (180.67,144.54) -- (104.79, 43.36);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (105.55, 44.37) -- (104.79, 43.36);

\path[draw=drawColor,line width= 1.2pt,line join=round,line cap=round] (105.66, 50.54) --
	(104.79, 43.36) --
	(111.44, 46.20);

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (148.73, 91.66) {$P_{uw^\perp}$};
\definecolor{fillColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (180.67,144.54) circle (  2.25);
\definecolor{drawColor}{RGB}{0,0,255}
\definecolor{fillColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (104.79, 43.36) circle (  2.25);
\end{scope}
\end{tikzpicture}


==> tikzR/weightedVariogram/bias_variance.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (289.08,289.08);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 57.15, 61.20) -- (255.93, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 57.15, 61.20) -- ( 57.15, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (106.85, 61.20) -- (106.85, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (156.54, 61.20) -- (156.54, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (206.23, 61.20) -- (206.23, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (255.93, 61.20) -- (255.93, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 57.15, 39.60) {3.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (106.85, 39.60) {4.0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (156.54, 39.60) {4.5};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (206.23, 39.60) {5.0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (255.93, 39.60) {5.5};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 67.82) -- ( 49.20,233.26);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 67.82) -- ( 43.20, 67.82);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,109.18) -- ( 43.20,109.18);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,150.54) -- ( 43.20,150.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,191.90) -- ( 43.20,191.90);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,233.26) -- ( 43.20,233.26);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 67.82) {0.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,109.18) {0.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,150.54) {1.0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,191.90) {1.5};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,233.26) {2.0};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(263.88, 61.20) --
	(263.88,239.88) --
	( 49.20,239.88) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (156.54, 15.60) {Squared Bias};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80,150.54) {Variance};
\end{scope}
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (263.88,239.88);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (694.49, 70.56) -- (607.43, 71.97);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (595.43, 72.22) -- (494.09, 74.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (482.11, 75.41) -- (372.42, 81.98);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (360.47, 82.99) -- (346.81, 84.47);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (334.90, 85.97) -- (319.37, 88.18);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (307.51, 90.05) -- (289.79, 93.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (277.95, 95.11) -- (251.77, 99.49);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (240.00,101.83) -- (215.23,107.52);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (204.08,111.67) -- (192.56,117.75);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (181.67,122.74) -- (174.92,125.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (164.71,131.39) -- (156.26,138.37);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (147.26,146.30) -- (133.68,159.07);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (126.61,168.54) -- (117.99,185.75);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (115.22,197.11) -- (112.11,430.44);
\definecolor{fillColor}{RGB}{0,0,255}

\path[fill=fillColor] (700.49, 70.46) circle (  2.25);

\path[fill=fillColor] (601.43, 72.06) circle (  2.25);

\path[fill=fillColor] (488.09, 75.05) circle (  2.25);

\path[fill=fillColor] (366.43, 82.34) circle (  2.25);

\path[fill=fillColor] (340.84, 85.12) circle (  2.25);

\path[fill=fillColor] (313.43, 89.03) circle (  2.25);

\path[fill=fillColor] (283.87, 94.12) circle (  2.25);

\path[fill=fillColor] (245.85,100.48) circle (  2.25);

\path[fill=fillColor] (209.38,108.87) circle (  2.25);

\path[fill=fillColor] (187.25,120.55) circle (  2.25);

\path[fill=fillColor] (169.34,127.57) circle (  2.25);

\path[fill=fillColor] (151.63,142.19) circle (  2.25);

\path[fill=fillColor] (129.30,163.18) circle (  2.25);

\path[fill=fillColor] (115.30,191.11) circle (  2.25);

\path[fill=fillColor] (112.03,436.44) circle (  2.25);
\definecolor{drawColor}{RGB}{160,32,240}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (400.38, 78.27) -- (355.72, 81.04);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (343.76, 82.01) -- (295.25, 86.90);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (283.39, 88.63) -- (231.47, 98.60);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (219.81,101.40) -- (217.75,102.00);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (206.30,105.58) -- (203.48,106.53);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (192.23,110.68) -- (188.81,112.05);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (177.97,117.16) -- (174.70,118.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (164.91,125.75) -- (161.79,128.46);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (153.99,137.43) -- (150.12,143.34);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (144.36,153.83) -- (143.80,155.09);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (140.10,166.43) -- (138.91,172.16);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (137.17,184.01) -- (135.98,197.65);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (135.85,209.62) -- (137.60,236.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (137.54,248.51) -- (119.52,485.85);
\definecolor{fillColor}{RGB}{160,32,240}

\path[fill=fillColor] (406.37, 81.40) --
	(409.40, 76.15) --
	(403.34, 76.15) --
	cycle;

\path[fill=fillColor] (349.73, 84.91) --
	(352.76, 79.66) --
	(346.70, 79.66) --
	cycle;

\path[fill=fillColor] (289.28, 91.00) --
	(292.31, 85.75) --
	(286.25, 85.75) --
	cycle;

\path[fill=fillColor] (225.58,103.24) --
	(228.61, 97.99) --
	(222.55, 97.99) --
	cycle;

\path[fill=fillColor] (211.99,107.16) --
	(215.02,101.91) --
	(208.96,101.91) --
	cycle;

\path[fill=fillColor] (197.80,111.94) --
	(200.83,106.69) --
	(194.77,106.69) --
	cycle;

\path[fill=fillColor] (183.24,117.79) --
	(186.27,112.54) --
	(180.21,112.54) --
	cycle;

\path[fill=fillColor] (169.43,125.30) --
	(172.46,120.06) --
	(166.40,120.06) --
	cycle;

\path[fill=fillColor] (157.27,135.91) --
	(160.30,130.66) --
	(154.24,130.66) --
	cycle;

\path[fill=fillColor] (146.83,151.86) --
	(149.86,146.62) --
	(143.80,146.62) --
	cycle;

\path[fill=fillColor] (141.33,164.05) --
	(144.36,158.80) --
	(138.30,158.80) --
	cycle;

\path[fill=fillColor] (137.69,181.54) --
	(140.72,176.29) --
	(134.66,176.29) --
	cycle;

\path[fill=fillColor] (135.46,207.13) --
	(138.49,201.88) --
	(132.43,201.88) --
	cycle;

\path[fill=fillColor] (137.99,246.03) --
	(141.02,240.78) --
	(134.96,240.78) --
	cycle;

\path[fill=fillColor] (119.07,495.34) --
	(122.10,490.09) --
	(116.04,490.09) --
	cycle;
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (505.85, 73.75) -- (442.54, 75.84);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (430.56, 76.38) -- (360.33, 80.38);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (348.38, 81.42) -- (271.80, 90.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (259.94, 92.19) -- (252.36, 93.54);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (240.58, 95.81) -- (231.69, 97.65);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (219.98,100.26) -- (209.90,102.67);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (198.35,105.88) -- (188.73,108.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (177.61,113.36) -- (169.18,117.45);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (159.09,123.81) -- (151.14,130.16);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (142.33,138.28) -- (140.65,140.06);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (134.01,149.87) -- (131.81,154.61);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (127.93,165.90) -- (125.15,177.93);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (124.27,189.76) -- (126.19,213.95);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (126.33,225.93) -- (113.07,461.01);
\definecolor{fillColor}{RGB}{255,165,0}

\path[fill=fillColor] (509.60, 71.30) --
	(514.10, 71.30) --
	(514.10, 75.80) --
	(509.60, 75.80) --
	cycle;

\path[fill=fillColor] (434.30, 73.79) --
	(438.80, 73.79) --
	(438.80, 78.29) --
	(434.30, 78.29) --
	cycle;

\path[fill=fillColor] (352.09, 78.47) --
	(356.59, 78.47) --
	(356.59, 82.97) --
	(352.09, 82.97) --
	cycle;

\path[fill=fillColor] (263.59, 88.88) --
	(268.09, 88.88) --
	(268.09, 93.38) --
	(263.59, 93.38) --
	cycle;

\path[fill=fillColor] (244.21, 92.35) --
	(248.71, 92.35) --
	(248.71, 96.85) --
	(244.21, 96.85) --
	cycle;

\path[fill=fillColor] (223.56, 96.61) --
	(228.06, 96.61) --
	(228.06,101.11) --
	(223.56,101.11) --
	cycle;

\path[fill=fillColor] (201.81,101.81) --
	(206.31,101.81) --
	(206.31,106.31) --
	(201.81,106.31) --
	cycle;

\path[fill=fillColor] (180.76,108.49) --
	(185.26,108.49) --
	(185.26,112.99) --
	(180.76,112.99) --
	cycle;

\path[fill=fillColor] (161.53,117.82) --
	(166.03,117.82) --
	(166.03,122.32) --
	(161.53,122.32) --
	cycle;

\path[fill=fillColor] (144.20,131.66) --
	(148.70,131.66) --
	(148.70,136.16) --
	(144.20,136.16) --
	cycle;

\path[fill=fillColor] (134.28,142.18) --
	(138.78,142.18) --
	(138.78,146.68) --
	(134.28,146.68) --
	cycle;

\path[fill=fillColor] (127.04,157.81) --
	(131.54,157.81) --
	(131.54,162.31) --
	(127.04,162.31) --
	cycle;

\path[fill=fillColor] (121.54,181.52) --
	(126.04,181.52) --
	(126.04,186.02) --
	(121.54,186.02) --
	cycle;

\path[fill=fillColor] (124.42,217.69) --
	(128.92,217.69) --
	(128.92,222.19) --
	(124.42,222.19) --
	cycle;

\path[fill=fillColor] (110.49,464.76) --
	(114.99,464.76) --
	(114.99,469.26) --
	(110.49,469.26) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (179.40,239.88) rectangle (263.88,179.88);
\definecolor{fillColor}{RGB}{0,0,255}

\path[fill=fillColor] (192.80,215.88) circle (  2.25);
\definecolor{fillColor}{RGB}{160,32,240}

\path[fill=fillColor] (192.80,207.38) --
	(195.83,202.13) --
	(189.77,202.13) --
	cycle;
\definecolor{fillColor}{RGB}{255,165,0}

\path[fill=fillColor] (190.55,189.63) --
	(195.05,189.63) --
	(195.05,194.13) --
	(190.55,194.13) --
	cycle;

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (221.64,227.88) {Weighting Scheme};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.80,212.44) {Equal};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.80,200.44) {Radial};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.80,188.44) {Radial CDF};
\definecolor{drawColor}{RGB}{190,190,190}

\path[draw=drawColor,line width= 0.4pt,dash pattern=on 4pt off 4pt ,line join=round,line cap=round] ( 49.20,214.85) -- (263.88, 36.17);
\end{scope}
\end{tikzpicture}


==> tikzR/weightedVariogram/mse_vs_p.tex <==
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (289.08,289.08);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 57.15, 61.20) -- (222.80, 61.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 57.15, 61.20) -- ( 57.15, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 98.56, 61.20) -- ( 98.56, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (139.98, 61.20) -- (139.98, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (181.39, 61.20) -- (181.39, 55.20);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (222.80, 61.20) -- (222.80, 55.20);

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 57.15, 39.60) {0.75};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 98.56, 39.60) {0.80};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (139.98, 39.60) {0.85};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (181.39, 39.60) {0.90};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (222.80, 39.60) {0.95};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 95.48) -- ( 49.20,233.10);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 95.48) -- ( 43.20, 95.48);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,129.89) -- ( 43.20,129.89);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,164.29) -- ( 43.20,164.29);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,198.69) -- ( 43.20,198.69);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20,233.10) -- ( 43.20,233.10);

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80, 95.48) {6};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,129.89) {7};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,164.29) {8};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,198.69) {9};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 34.80,233.10) {10};

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 49.20, 61.20) --
	(263.88, 61.20) --
	(263.88,239.88) --
	( 49.20,239.88) --
	cycle;
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (289.08,289.08);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (156.54, 15.60) {Threshold p};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at ( 10.80,150.54) {MSE};
\end{scope}
\begin{scope}
\path[clip] ( 49.20, 61.20) rectangle (263.88,239.88);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 61.81,229.48) -- ( 93.91,203.42);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (102.98,195.58) -- (135.55,165.70);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (144.34,157.53) -- (177.02,126.68);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (209.95, 94.16) -- (210.80, 93.07);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (218.54, 83.91) -- (218.77, 83.66);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (248.14, 86.76) -- (255.44,175.49);
\definecolor{fillColor}{RGB}{0,0,255}

\path[fill=fillColor] ( 57.15,233.26) circle (  2.25);

\path[fill=fillColor] ( 98.56,199.64) circle (  2.25);

\path[fill=fillColor] (139.98,161.65) circle (  2.25);

\path[fill=fillColor] (181.39,122.56) circle (  2.25);

\path[fill=fillColor] (189.67,114.86) circle (  2.25);

\path[fill=fillColor] (197.95,106.99) circle (  2.25);

\path[fill=fillColor] (206.23, 98.87) circle (  2.25);

\path[fill=fillColor] (214.52, 88.35) circle (  2.25);

\path[fill=fillColor] (222.80, 79.21) circle (  2.25);

\path[fill=fillColor] (231.08, 76.40) circle (  2.25);

\path[fill=fillColor] (235.22, 73.11) circle (  2.25);

\path[fill=fillColor] (239.36, 73.05) circle (  2.25);

\path[fill=fillColor] (243.51, 74.03) circle (  2.25);

\path[fill=fillColor] (247.65, 80.78) circle (  2.25);

\path[fill=fillColor] (255.93,181.47) circle (  2.25);
\definecolor{drawColor}{RGB}{160,32,240}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 62.65,132.13) -- ( 93.07,118.80);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (104.05,113.96) -- (134.49,100.43);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (145.53, 95.72) -- (175.84, 83.30);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (244.92, 98.78) -- (246.23,104.14);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (248.16,115.95) -- (255.42,200.92);
\definecolor{fillColor}{RGB}{160,32,240}

\path[fill=fillColor] ( 57.15,138.04) --
	( 60.18,132.79) --
	( 54.12,132.79) --
	cycle;

\path[fill=fillColor] ( 98.56,119.89) --
	(101.59,114.65) --
	( 95.53,114.65) --
	cycle;

\path[fill=fillColor] (139.98,101.50) --
	(143.01, 96.25) --
	(136.94, 96.25) --
	cycle;

\path[fill=fillColor] (181.39, 84.52) --
	(184.42, 79.28) --
	(178.36, 79.28) --
	cycle;

\path[fill=fillColor] (189.67, 81.45) --
	(192.70, 76.20) --
	(186.64, 76.20) --
	cycle;

\path[fill=fillColor] (197.95, 78.52) --
	(200.98, 73.27) --
	(194.92, 73.27) --
	cycle;

\path[fill=fillColor] (206.23, 75.91) --
	(209.26, 70.66) --
	(203.20, 70.66) --
	cycle;

\path[fill=fillColor] (214.52, 74.25) --
	(217.55, 69.00) --
	(211.49, 69.00) --
	cycle;

\path[fill=fillColor] (222.80, 74.44) --
	(225.83, 69.19) --
	(219.77, 69.19) --
	cycle;

\path[fill=fillColor] (231.08, 77.45) --
	(234.11, 72.20) --
	(228.05, 72.20) --
	cycle;

\path[fill=fillColor] (235.22, 80.60) --
	(238.25, 75.36) --
	(232.19, 75.36) --
	cycle;

\path[fill=fillColor] (239.36, 86.60) --
	(242.39, 81.35) --
	(236.33, 81.35) --
	cycle;

\path[fill=fillColor] (243.51, 96.45) --
	(246.54, 91.20) --
	(240.48, 91.20) --
	cycle;

\path[fill=fillColor] (247.65,113.47) --
	(250.68,108.23) --
	(244.62,108.23) --
	cycle;

\path[fill=fillColor] (255.93,210.40) --
	(258.96,205.15) --
	(252.90,205.15) --
	cycle;
\definecolor{drawColor}{RGB}{255,165,0}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] ( 62.29,166.14) -- ( 93.43,147.32);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (103.62,140.98) -- (134.92,120.94);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (145.04,114.48) -- (176.32, 94.61);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (245.01, 86.48) -- (246.14, 90.87);

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round] (248.15,102.66) -- (255.42,188.42);
\definecolor{fillColor}{RGB}{255,165,0}

\path[fill=fillColor] ( 54.90,167.00) --
	( 59.40,167.00) --
	( 59.40,171.50) --
	( 54.90,171.50) --
	cycle;

\path[fill=fillColor] ( 96.31,141.97) --
	(100.81,141.97) --
	(100.81,146.47) --
	( 96.31,146.47) --
	cycle;

\path[fill=fillColor] (137.73,115.45) --
	(142.23,115.45) --
	(142.23,119.95) --
	(137.73,119.95) --
	cycle;

\path[fill=fillColor] (179.14, 89.14) --
	(183.64, 89.14) --
	(183.64, 93.64) --
	(179.14, 93.64) --
	cycle;

\path[fill=fillColor] (187.42, 83.87) --
	(191.92, 83.87) --
	(191.92, 88.37) --
	(187.42, 88.37) --
	cycle;

\path[fill=fillColor] (195.70, 78.50) --
	(200.20, 78.50) --
	(200.20, 83.00) --
	(195.70, 83.00) --
	cycle;

\path[fill=fillColor] (203.98, 73.12) --
	(208.48, 73.12) --
	(208.48, 77.62) --
	(203.98, 77.62) --
	cycle;

\path[fill=fillColor] (212.27, 68.61) --
	(216.77, 68.61) --
	(216.77, 73.11) --
	(212.27, 73.11) --
	cycle;

\path[fill=fillColor] (220.55, 65.82) --
	(225.05, 65.82) --
	(225.05, 70.32) --
	(220.55, 70.32) --
	cycle;

\path[fill=fillColor] (228.83, 65.57) --
	(233.33, 65.57) --
	(233.33, 70.07) --
	(228.83, 70.07) --
	cycle;

\path[fill=fillColor] (232.97, 66.50) --
	(237.47, 66.50) --
	(237.47, 71.00) --
	(232.97, 71.00) --
	cycle;

\path[fill=fillColor] (237.11, 70.48) --
	(241.61, 70.48) --
	(241.61, 74.98) --
	(237.11, 74.98) --
	cycle;

\path[fill=fillColor] (241.26, 78.42) --
	(245.76, 78.42) --
	(245.76, 82.92) --
	(241.26, 82.92) --
	cycle;

\path[fill=fillColor] (245.40, 94.43) --
	(249.90, 94.43) --
	(249.90, 98.93) --
	(245.40, 98.93) --
	cycle;

\path[fill=fillColor] (253.68,192.15) --
	(258.18,192.15) --
	(258.18,196.65) --
	(253.68,196.65) --
	cycle;
\definecolor{drawColor}{RGB}{0,0,0}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.4pt,line join=round,line cap=round,fill=fillColor] (179.40,239.88) rectangle (263.88,179.88);
\definecolor{fillColor}{RGB}{0,0,255}

\path[fill=fillColor] (192.80,215.88) circle (  2.25);
\definecolor{fillColor}{RGB}{160,32,240}

\path[fill=fillColor] (192.80,207.38) --
	(195.83,202.13) --
	(189.77,202.13) --
	cycle;
\definecolor{fillColor}{RGB}{255,165,0}

\path[fill=fillColor] (190.55,189.63) --
	(195.05,189.63) --
	(195.05,194.13) --
	(190.55,194.13) --
	cycle;

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  1.00] at (221.64,227.88) {Weighting Scheme};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.80,212.44) {Equal};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.80,200.44) {Radial};

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  1.00] at (201.80,188.44) {Radial CDF};
\end{scope}
\end{tikzpicture}

